Notes on the post-bounce background dynamics in bouncing cosmologies

We investigate the post-bounce background dynamics in a certain class of single bounce scenarios studied in the literature, in which the cosmic bounce is driven by a scalar field with negative exponential potential such as the ekpyrotic potential. We show that those models can actually lead to cyclic evolutions with repeated bounces. These cyclic evolutions, however, do not account for the currently observed late-time accelerated expansion and hence are not cosmologically viable. In this respect we consider a new kind of cyclic model proposed recently and derive some cosmological constraints on this model.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%              LaTeX macros -- Ioannis Papadimitriou v. 09.12.2015
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Shortcuts


\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\comment}[1]{\textcolor{blue!60}{[#1]}} %requires xcolor

\def \bib{\bibitem}
\def\){\right)}
\def\({\left( }
\def\]{\right] }
\def\[{\left[ }
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

\def\NO{\nonumber}
\def\nonu{\nonumber \\}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}


\def\bal#1\eal{\begin{align}#1\end{align}}
\def\bala#1\eala{\begin{align*}#1\end{align*}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\def\bald{\begin{aligned}}
\def\eald{\end{aligned}}

\def\bsub{\begin{subequations}}
\def\esub{\end{subequations}}



\def\beqx{\begin{displaymath}}
\def\eeqx{\end{displaymath}}

\newcommand{\bmat}{\left(\begin{array}}
\newcommand{\emat}{\end{array}\right)}

%\renewcommand{\theequation}{\thesection.\arabic{equation}}


% New environments

\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{conjecture}{Conjecture}[section]

% Abbreviations for Greek letters

\def\a{\alpha}
\def\b{\beta}
\def\c{\chi}
\def\d{\delta}
\def\e{\epsilon}
\def\f{\phi}
\def\g{\gamma}
\def\h{\eta}
%\def\i{\iota} %conflicts with accents in Latin input
\def\j{\psi}
\def\k{\kappa}
\def\l{\lambda}
\def\m{\mu}
\def\n{\nu}
\def\o{\omega}
    \def\om{\omega}
\def\p{\pi}
\def\q{\theta}
    \def\th{\theta}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
%\def\u{\upsilon}
\def\x{\xi}
\def\z{\zeta}
\def\D{\Delta}
\def\F{\Phi}
\def\G{\Gamma}
\def\J{\Psi}
\def\L{\Lambda}
\def\O{\Omega}
    \def\Om{\Omega}
\def\P{\Pi}
\def\Q{\Theta}
    \def\Th{\Theta}
\def\S{\Sigma}
\def\U{\Upsilon}
\def\X{\Xi}

% Varletters

\def\ve{\varepsilon}
\def\vr{\varrho}
\def\vs{\varsigma}
\def\vq{\vartheta}
    \def\vth{\vartheta}
\def\tvf{\tilde{\varphi}}
\def\vf{\varphi}
    \def\vphi{\varphi}

% Greek bb letters -- requires \usepackage[bbgreekl]{mathbbol}

\def\ba{\bbalpha}
\def\bk{\bbkappa}
\def\bg{\bbgamma}
\def\bd{\bbdelta}
%\def\be{\bbepsilon}
\def\bs{\bbsigma}

% Calligraphic letters

\def\ca{{\cal A}}
\def\cb{{\cal B}}
\def\cc{{\cal C}}
\def\cd{{\cal D}}
\def\ce{{\cal E}}
\def\cf{{\cal F}}
\def\cg{{\cal G}}
\def\ch{{\cal H}}
\def\ci{{\cal I}}
\def\cj{{\cal J}}
\def\ck{{\cal K}}
\def\cl{{\cal L}}
\def\cm{{\cal M}}
\def\cn{{\cal N}}
\def\co{{\cal O}}
\def\cp{{\cal P}}
\def\cq{{\cal Q}}
\def\car{{\cal R}}
\def\cs{{\cal S}}
\def\ct{{\cal T}}
\def\cu{{\cal U}}
\def\cv{{\cal V}}
\def\cw{{\cal W}}
\def\cx{{\cal X}}
\def\cy{{\cal Y}}
\def\cz{{\cal Z}}


% Mathfrak fonts

\def\fA{{\mathfrak A}}
\def\fB{{\mathfrak B}}
\def\fC{{\mathfrak C}}
\def\fD{{\mathfrak D}}
\def\fE{{\mathfrak E}}
\def\fF{{\mathfrak F}}
\def\fG{{\mathfrak G}}
\def\fH{{\mathfrak H}}
\def\fI{{\mathfrak I}}
\def\fJ{{\mathfrak J}}
\def\fK{{\mathfrak K}}

% Accents and foreign (in text):

% Fonts

\def\Sc#1{{\hbox{\sc #1}}}      % script for single characters in equations
\def\Sf#1{{\hbox{\sf #1}}}      % sans serif for single characters in equations
\def\mb#1{\mbox{\boldmath $#1$}}% bold math character
\def\mf#1{\ensuremath{\mathfrak{#1}}} %mathfrak
\def\bb#1{\ensuremath{\mathbb{#1}}} %mathbb

% Math symbols

%\newcommand{\dd}{\mathrm{d}}
\def\slpa{\slash{\pa}}                         % slashed partial derivative
\def\slin{\SLLash{\in}}                                 % slashed in-sign
\def\bo{{\raise-.3ex\hbox{\large$\Box$}}}               % D'Alembertian
\def\cbo{\Sc [}                                         % curly "
\def\pa{\partial}                                       % curly d
\def\de{\nabla}                                         % del
\def\dell{\nabla}                                       % hi ho the dairy-o
\def\su{\sum}                                           % summation
\def\pr{\prod}                                          % product
\def\iff{\leftrightarrow}                               % <-->
\def\conj{{\hbox{\large *}}}                            % complex conjugate
\def\ltap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$<$}}   % < or ~
\def\gtap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$>$}}   % > or ~
\def\face{{\raise.2ex\hbox{$\displaystyle \bigodot$}\mskip-2.2mu \llap {$\ddot
        \smile$}}}                                   % happy face
\def\dg{\dagger}                                     % hermitian conjugate
\def\ddg{\ddagger}                                   % double dagger
\def\trans{\mbox{\scri T}}                           % T for transposition
\def\>{\rangle}                                      %right angle
\def\<{\langle}                                      %left angle

% Math stuff with one argument

\def\sp#1{{}^{#1}}                                   % superscript (unaligned)
\def\sb#1{{}_{#1}}                                   % sub"
\newcommand{\sub}[1]{\phantom{}_{(#1)}\phantom{}}    % subscript in ( )
\def\oldsl#1{\rlap/#1}                               % poor slash
\def\slash#1{\rlap{\hbox{$\mskip 1 mu /$}}#1}        % good slash for lower case
\def\Slash#1{\rlap{\hbox{$\mskip 3 mu /$}}#1}        % " upper
\def\SLash#1{\rlap{\hbox{$\mskip 4.5 mu /$}}#1}      % " fat stuff (e.g., M)
\def\SLLash#1{\rlap{\hbox{$\mskip 6 mu /$}}#1}       % slash for no-in sign
\def\wt#1{\widetilde{#1}}                            % big tilde
\def\Hat#1{\widehat{#1}}                             % big hat
\def\lbar#1{\ensuremath{\overline{#1}}}              % big bar

\def\VEV#1{\left\langle #1\right\rangle}             % < >
\def\abs#1{\left| #1\right|}                         % | |
\def\leftrightarrowfill{$\mathsurround=0pt \mathord\leftarrow \mkern-6mu
        \cleaders\hbox{$\mkern-2mu \mathord- \mkern-2mu$}\hfill
        \mkern-6mu \mathord\rightarrow$}        % <--> double differential
\def\dvec#1{\vbox{\ialign{##\crcr
        \leftrightarrowfill\crcr\noalign{\kern-1pt\nointerlineskip}
        $\hfil\displaystyle{#1}\hfil$\crcr}}}           % <--> accent
\def\dt#1{{\buildrel {\hbox{\LARGE .}} \over {#1}}}     % dot-over for sp/sb
\def\dtt#1{{\buildrel \bullet \over {#1}}}              % alternate "
\def\der#1{{\pa \over \pa {#1}}}                        % partial derivative
\def\fder#1{{\d \over \d {#1}}}                         % functional derivative
\def\tr{{\rm tr \,}}                                    % trace
\def\Tr{{\rm Tr \,}}                                    % Trace
\def\diag{{\rm diag \,}}                                % diagonal
\def\Re{{\rm Re\,}}                                     % Real part
\def\Im{{\rm Im\,}}                                     % Imaginary part

% Math stuff with more than one argument

\def\partder#1#2{{\partial #1\over\partial #2}}        % partial derivative of
\def\parvar#1#2{{\d #1\over \d #2}}                    % variation of
\def\secder#1#2#3{{\partial^2 #1\over\partial #2 \partial #3}}  % second "
\def\on#1#2{\mathop{\null#2}\limits^{#1}}              % arbitrary accent
\def\bvec#1{\on\leftarrow{#1}}                         % backward vector accent
\def\oover#1{\on\circ{#1}}                             % circle accent

% Physics related

\def\Deq#1{\mbox{$D$=#1}}                               % Dimension
\def\Neq#1{\mbox{$cn$=#1}}                              % SUSY
\newcommand{\ampl}[2]{{\cal M}\left( #1 \to #2 \right)} % Scattering amplitude

% Abbreviations for journals

\def\NPB#1#2#3{Nucl. Phys. B {\bf #1} (19#2) #3}
\def\PLB#1#2#3{Phys. Lett. B {\bf #1} (19#2) #3}
\def\PLBold#1#2#3{Phys. Lett. {\bf #1}B (19#2) #3}
\def\PRD#1#2#3{Phys. Rev. D {\bf #1} (19#2) #3}
\def\PRL#1#2#3{Phys. Rev. Lett. {\bf #1} (19#2) #3}
\def\PRT#1#2#3{Phys. Rep. {\bf #1} C (19#2) #3}
\def\MODA#1#2#3{Mod. Phys. Lett.  {\bf #1} (19#2) #3}

% Miscellaneous

\def\norder{\raisebox{-.13cm}{\ensuremath{\circ}}\hspace{-.174cm}\raisebox{.13cm}{\ensuremath{\circ}}}
\def\bz{\bar{z}}
\def\bw{\bar{w}}
\def\-{\hphantom{-}}
\newcommand{\dd}{\mbox{d}}
\newcommand{\scr}{\scriptscriptstyle}
\newcommand{\scri}{\scriptsize}
\def\rand#1{\marginpar{\tiny #1}}               % Randbemerkung
\newcommand{\rstar}{\rand{\bf\large *}}
\newcommand{\rup}{\rand{$\uparrow$}}
\newcommand{\rdown}{\rand{$\downarrow$}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Song's definitions

\def\labD {\overleftarrow{\bb D}}
\def\slabD {\overleftarrow{\slashed{\bb D}}}
\newcommand\encircle[1]{%
  \tikz[baseline=(X.base)] 
    \node (X) [draw, shape=circle, inner sep=0] {\strut #1};}

\def\unit {\mathds{1}}
\def\tnabla {\wt\nabla}
\def\sfD {\slashed\fD}
\def\spa {\slashed\pa}

